Entropy-Compatible Barrier Schemes for Diffusive FENE Flows

FENE-type conformation-tensor models impose a finite-extensibility constraint that is absent from Oldroyd--B flow: the conformation tensor must satisfy $\CC\succ0$ and $\tr\CC<L^2$. Positive definiteness alone is therefore insufficient, since a numerical state can remain positive while crossing the singular trace barrier. Even a trace-preserving logarithmic parametrization is not enough by itself: high-order reconstruction can remain inside the finite-extensibility domain while injecting artificial FENE entropy. We develop and analyze a barrier-preserving entropy-compatible discretization for FENE-P type flows with polymer center-of-mass molecular diffusion and for trace-singular FENE-family closures with the same entropy structure. The method combines a trace-barrier free energy, a finite-extensibility logarithmic parametrization, a least-damping entropy-compatible barrier-log reconstruction, molecular diffusion paired with the barrier entropy variable, compatible quadrature for polymeric work, and a scaled FENE stress variable for the small-Weissenberg limit. For admissible discrete states we prove finite-extensibility preservation at entropy quadrature points, existence and bisection computability of the maximal entropy-admissible reconstruction parameter, a fully discrete free-energy inequality with relaxation and molecular-diffusion barrier dissipation, a quantitative AP stress closure, and a fixed-discretization Newtonian limit. A conditional relative-entropy estimate is derived on compact subsets of the finite-extensibility domain. Numerical diagnostics verify barrier preservation, entropy-compatible reconstruction, energy decay, AP closure, coupled velocity--pressure--stress accuracy, and high-Weissenberg robustness near the trace constraint.

==> data_reconstruction_comparison_table.tex <==
\begin{tabular}{ccccccc}
\toprule
$a$ & log $\tr C/b$ & repair $\Delta\Phi$ & barrier-log $\tr C/b$ & barrier-log $\Delta\Phi$ & entropy-log $\Delta\Phi$ & $\theta_\star$ \\
\midrule
0.25 & 1.060 & 210.438 & 0.898 & 3.117 & 0.100 & 0.035 \\
0.50 & 1.302 & 210.657 & 0.916 & 6.658 & 0.100 & 0.017 \\
0.75 & 1.625 & 210.908 & 0.931 & 10.563 & 0.100 & 0.012 \\
1.00 & 2.055 & 211.185 & 0.945 & 14.767 & 0.100 & 8.64E-3 \\
1.25 & 2.622 & 211.480 & 0.956 & 19.212 & 0.100 & 6.91E-3 \\
1.50 & 3.371 & 211.790 & 0.966 & 23.847 & 0.100 & 5.76E-3 \\
\bottomrule
\end{tabular}

